Code Reasoning for Software Engineering Tasks: A Survey and A Call to Action

The rise of large language models (LLMs) has led to dramatic improvements across a wide range of natural language tasks. Their performance on certain tasks can be further enhanced by incorporating test-time reasoning techniques. These inference-time advances have been adopted into the code domain, enabling complex software engineering (SWE) tasks such as code generation, test generation and issue resolution. However, the impact of different reasoning techniques on code-centric SWE tasks has not been systematically explored. In this work, we survey code reasoning techniques that underpin these capabilities, with a focus on test-time compute and inference-time reasoning paradigms. We examine a variety of code-specific reasoning methods and progressively build up to SWE agents, which combine planning, tool use, and multi-step interaction. We also compare the impact of different techniques on coding tasks, highlighting their relative importance and outlining open challenges and future research directions. Across commonly used models and benchmarks, we find that approaches exploiting code-specific signals (e.g., structure and execution feedback) are frequently associated with improved performance, motivating a dedicated study of code reasoning beyond natural-language reasoning.

==> sections/results-obs-define-patterns.tex <==
\usetikzlibrary{patterns,patterns.meta}

\definecolor{OrangeBase}{HTML}{F57C00}
\definecolor{BlueSoft}{HTML}{4796E5}
\definecolor{Blue60}{HTML}{6699FF}

\tikzset{
  orangePattern3/.style={
    fill=OrangeBase!65,
    draw=OrangeBase!80!black,
    postaction={pattern=crosshatch, pattern color=black}
  },
  redPatternDarkDots/.style={
    fill=red!55!black,
    draw=red!70!black,
    postaction={pattern=dots, pattern color=red!20}
},
redPatternDarkLinesWest/.style={
    fill=red!60!black,
    draw=red!80!black,
    postaction={pattern=north west lines, pattern color=red!15}
},
redPatternMediumDotsDark/.style={
    fill=red!40,
    draw=red!70!black,
    postaction={pattern=dots, pattern color=red!85!black}
},
redPatternDarkCrosshatch/.style={
    fill=red!55!black,
    draw=red!75!black,
    postaction={pattern=crosshatch, pattern color=red!20}
},
redPatternLightHorizontal/.style={
    fill=red!25,
    draw=red!65!black,
    postaction={pattern=horizontal lines, pattern color=red!75!black}
},
redPatternLightCrosshatch/.style={
    fill=red!20,
    draw=red!60!black,
    postaction={pattern=crosshatch, pattern color=red!70!black}
},
redPatternDarkVertical/.style={
    fill=red!60!black,
    draw=red!80!black,
    postaction={pattern=vertical lines, pattern color=white!80!red}
},
  orangePattern7/.style={
    fill=OrangeBase!10,
    draw=OrangeBase!80!black,
    postaction={
      pattern=north west lines,
      pattern color=OrangeBase!90!black
    }
  },
  redWineCreamDots/.style={
    fill=red!55!purple!15,
    draw=red!70!purple!20,
    postaction={pattern=dots, pattern color=red!10!white}
},
  redPatternDarkWhiteLinesEast/.style={
    fill=red!50!black,
    draw=red!70!black,
    postaction={pattern=north east lines, pattern color=white}
},
  redPatternMediumHashNE/.style={
    fill=red!40,
    draw=red!80!black,
    postaction={pattern=north east lines, pattern color=red!90!black}
},
  redBurgundyWhiteGrid/.style={
    fill=red!65!black!15,
    draw=red!80!black,
    postaction={pattern=grid, pattern color=white!90}
},
  orangePattern5/.style={
    fill=OrangeBase!90,
    draw=OrangeBase!80!black
  },
  orangePattern5light/.style={
    fill=OrangeBase!35
  },
  orangePattern4/.style={
    fill=OrangeBase!75!black,
    draw=OrangeBase!80!black
  },
  orangePattern2/.style={
    fill=OrangeBase!40,
    draw=OrangeBase!80!black,
    postaction={pattern=north east lines, pattern color=OrangeBase!90!black}
  },
  bluePatternwhitelinesleft/.style={
    fill=blue!40,               
    draw=blue!80!black,         
    postaction={ pattern=north west lines, pattern color=white }
  },
  bluePurpleStripes/.style={
    fill=blue!40!black!10,                % bluish base tone
    draw=blue!80!black,                   % darker border
    postaction={
      pattern=north west lines,
      pattern color=purple!60!blue!30     % bluish purple stripes
    }
 },
 bluePurpleStripesBlackOpp/.style={
    fill=blue!40!black!10,          % same blue base
    draw=blue!80!black,             % same border
    postaction={
      pattern=north east lines,     % opposite direction
      pattern color=black           % black stripes
    }
},
bluePurpleStripesDark/.style={
    fill=blue!55!purple!10,        % bluer purplish base
    draw=blue!75!black,            % darker bluish border
    postaction={
      pattern=crosshatch,          % cross-hash pattern
      pattern color=blue!50!purple!30!blue   % dark bluish-purple hash
    }
},
darkGreenLightWest/.style={
    fill=green!70!black,           % dark green background
    draw=green!80!black,           % slightly darker border
    postaction={
      pattern=north west lines,    % lines slanting “west”
      pattern color=green!10!white % light greenish stripes
    },
},
lightGreenDarkEast/.style={
    fill=lime!25!white,            % light lime background
    draw=green!60!black,
    postaction={
      pattern=north east lines,    % lines slanting “east”
      pattern color=green!70!black % dark green stripes
    },
},
lightGreenSolid/.style={
    fill=lime!35!white,            % soft light green
    draw=green!50!black            % modest green border
},
limeGreenCrossDark/.style={
    fill=lime!60!green!15,         % lime-green base slightly toned by green
    draw=green!60!black,           % darker green border
    postaction={
      pattern=crosshatch,          % cross-hash pattern
      pattern color=green!70!black % dark green hash lines
    }
},
  bluePattern1/.style={
    fill=BlueSoft!95!black,
    draw=BlueSoft!95!black,
    postaction={pattern=crosshatch, pattern color=white}
  },
  bluePattern2/.style={
    fill=BlueSoft!40,
    draw=BlueSoft!80!black,
    postaction={pattern=north east lines, pattern color=BlueSoft!90!black}
  },
  bluePattern2Struct/.style={
    fill=Blue60!40,
    draw=Blue60!80!black,
    postaction={pattern=north east lines, pattern color=Blue60!90!black}
  },
  bluePattern3/.style={
    fill=BlueSoft!65,
    draw=BlueSoft!80!black,
    postaction={pattern=crosshatch, pattern color=black}
  },
  bluePattern4/.style={
    fill=BlueSoft!75!black,
    draw=BlueSoft!80!black
  },
  bluePattern5/.style={
    fill=BlueSoft!90,
    draw=BlueSoft!80!black
  },
  bluePattern6/.style={
    fill=BlueSoft!35,
    draw=BlueSoft!80!black
  },
  bluePattern8/.style={
    fill=BlueSoft!20,
    draw=BlueSoft!80!black,
    postaction={pattern=dots, pattern color=BlueSoft!90!black}
  },
  bluePattern9/.style={
    fill=BlueSoft!60,
    draw=BlueSoft!80!black,
    postaction={pattern=horizontal lines, pattern color=BlueSoft!90!black}
  }
}




==> sections/results-obs-exec.tex <==
% ===== Smaller demo plot: orange pattern variants (6 total) =====
\definecolor{OrangeBase}{HTML}{F57C00}

\tikzset{
  % 1. Dark bg + white dots
orangePattern1/.style={
  fill=OrangeBase!80!black,
  draw=OrangeBase!80!black,
  postaction={pattern={Dots[distance=2pt,radius=0.6pt]}, pattern color=white}
},
  % 2. Light bg + dark diagonal lines
  orangePattern2/.style={
    fill=OrangeBase!40,
    draw=OrangeBase!80!black,
    postaction={pattern=north east lines, pattern color=OrangeBase!90!black}
  },
  % 3. Medium bg + black crosshatch
  orangePattern3/.style={
    fill=OrangeBase!65,
    draw=OrangeBase!80!black,
    postaction={pattern=crosshatch, pattern color=black}
  },
  % 4. Solid bright orange (for contrast)
  orangePattern4/.style={
    fill=OrangeBase!75!black,
    draw=OrangeBase!80!black
  },
   orangePattern5/.style={
    fill=OrangeBase!90,
    draw=OrangeBase!80!black
  },
 orangePattern6/.style={
    fill=OrangeBase!35,
    draw=OrangeBase!80!black
  },
orangePattern7/.style={
  fill=OrangeBase!10,                % light orange background
  draw=OrangeBase!80!black,          % dark outline
  postaction={
    pattern=horizontal lines,        % overlay horizontal stripes
    pattern color=OrangeBase!90!black  % dark orange lines
  }
},

  orangePattern8/.style={
    fill=OrangeBase!20,
    draw=OrangeBase!80!black,
    postaction={pattern=dots, pattern color=OrangeBase!90!black}
  },
  % 6. Medium bg + horizontal lines
  orangePattern9/.style={
    fill=OrangeBase!60,
    draw=OrangeBase!80!black,
    postaction={pattern=horizontal lines, pattern color=OrangeBase!90!black}
  }
}

\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar=0pt,
  bar width=8pt,
  width=0.52\textwidth, height=4.4cm,
  ymin=0, ymax=100,
  ytick={0,20,40,60,80,100},
  symbolic x coords={P1,P2,P3,P4,P5,P6},
  xtick=data,
  grid=major,
  title={Six Orange Variants (solid + patterned)},
  legend style={at={(0.5,-0.20)}, anchor=north, legend columns=2,
    /tikz/every even column/.style={column sep=0.4cm}}
]
  % Bars
\addplot[orangePattern1] coordinates {(P3,72)};
\addplot[orangePattern2] coordinates {(P3,72)};
\addplot[orangePattern3] coordinates {(P3,72)};
\addplot[orangePattern4] coordinates {(P3,72)};
\addplot[orangePattern5] coordinates {(P3,72)};
\addplot[orangePattern6] coordinates {(P3,72)};
\addplot[orangePattern7] coordinates {(P3,72)};
\addplot[orangePattern8] coordinates {(P3,72)};
\addplot[orangePattern9] coordinates {(P3,72)};

\addlegendimage{ybar, orangePattern1}\addlegendentry{dark bg + white dots}
\addlegendimage{ybar, orangePattern2}\addlegendentry{light bg + dark lines}
\addlegendimage{ybar, orangePattern3}\addlegendentry{medium bg + crosshatch}
\addlegendimage{ybar, orangePattern4}\addlegendentry{solid bright orange}
\addlegendimage{ybar, orangePattern5}\addlegendentry{light bg + dark dots}
\addlegendimage{ybar, orangePattern6}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, orangePattern7}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, orangePattern8}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, orangePattern9}\addlegendentry{medium bg + horiz lines}

\end{axis}
\end{tikzpicture}
\caption{Six distinct orange fill styles for print and digital contrast.}
\end{figure}


==> sections/results-obs-inf.tex <==
% ===== Smaller demo plot: green pattern variants (6 total) =====
\definecolor{GreenBase}{HTML}{6CC644}

\tikzset{
  % 1. Dark bg + white dots
greenPattern1/.style={
  fill=GreenBase!80!black,
  draw=GreenBase!80!black,
  postaction={pattern={Dots[distance=2pt,radius=0.6pt]}, pattern color=white}
},
  % 2. Light bg + dark diagonal lines
  greenPattern2/.style={
    fill=GreenBase!40,
    draw=GreenBase!80!black,
    postaction={pattern=north east lines, pattern color=GreenBase!90!black}
  },
  % 3. Medium bg + black crosshatch
  greenPattern3/.style={
    fill=GreenBase!65,
    draw=GreenBase!80!black,
    postaction={pattern=crosshatch, pattern color=black}
  },
  % 4. Solid bright green (for contrast)
  greenPattern4/.style={
    fill=GreenBase!75!black,
    draw=GreenBase!80!black
  },
   greenPattern5/.style={
    fill=GreenBase!90,
    draw=GreenBase!80!black
  },
 greenPattern6/.style={
    fill=GreenBase!35,
    draw=GreenBase!80!black
  },
greenPattern7/.style={
  fill=GreenBase!10,                % light green background
  draw=GreenBase!80!black,          % dark outline
  postaction={
    pattern=horizontal lines,        % overlay horizontal stripes
    pattern color=GreenBase!90!black  % dark green lines
  }
},

  greenPattern8/.style={
    fill=GreenBase!20,
    draw=GreenBase!80!black,
    postaction={pattern=dots, pattern color=GreenBase!90!black}
  },
  % 6. Medium bg + horizontal lines
  greenPattern9/.style={
    fill=GreenBase!60,
    draw=GreenBase!80!black,
    postaction={pattern=horizontal lines, pattern color=GreenBase!90!black}
  }
}

\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar=0pt,
  bar width=8pt,
  width=0.52\textwidth, height=4.4cm,
  ymin=0, ymax=100,
  ytick={0,20,40,60,80,100},
  symbolic x coords={P1,P2,P3,P4,P5,P6},
  xtick=data,
  grid=major,
  title={Six Green Variants (solid + patterned)},
  legend style={at={(0.5,-0.20)}, anchor=north, legend columns=2,
    /tikz/every even column/.style={column sep=0.4cm}}
]
  % Bars
\addplot[greenPattern1] coordinates {(P3,72)};
\addplot[greenPattern2] coordinates {(P3,72)};
\addplot[greenPattern3] coordinates {(P3,72)};
\addplot[greenPattern4] coordinates {(P3,72)};
\addplot[greenPattern5] coordinates {(P3,72)};
\addplot[greenPattern6] coordinates {(P3,72)};
\addplot[greenPattern7] coordinates {(P3,72)};
\addplot[greenPattern8] coordinates {(P3,72)};
\addplot[greenPattern9] coordinates {(P3,72)};

\addlegendimage{ybar, greenPattern1}\addlegendentry{dark bg + white dots}
\addlegendimage{ybar, greenPattern2}\addlegendentry{light bg + dark lines}
\addlegendimage{ybar, greenPattern3}\addlegendentry{medium bg + crosshatch}
\addlegendimage{ybar, greenPattern4}\addlegendentry{solid bright green}
\addlegendimage{ybar, greenPattern5}\addlegendentry{light bg + dark dots}
\addlegendimage{ybar, greenPattern6}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, greenPattern7}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, greenPattern8}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, greenPattern9}\addlegendentry{medium bg + horiz lines}

\end{axis}
\end{tikzpicture}
\caption{Six distinct green fill styles for print and digital contrast.}
\end{figure}


==> sections/results-obs-plan-cot.tex <==
% Deep, strong blue (good for outlines / emphasis)
\definecolor{BlueDeep}{HTML}{003f5c}

% Medium saturated blue — “primary bar color”
\definecolor{BlueMid}{HTML}{0074D9}

% Soft / muted blue for contrast against BlueMid
\definecolor{BlueSoft}{HTML}{4796E5}

% Very light blue (for fill with pattern overlays)
\definecolor{BlueLight}{HTML}{B3D4FF}

% Blue with slight turquoise lean (good to break monotony)
\definecolor{BlueTeal}{HTML}{0096A7}

% Navy — excellent for text legends / bold emphasis
\definecolor{BlueNavy}{HTML}{001F3F}
\definecolor{Blue60}{HTML}{6699FF}


\tikzset{
  % 1. Dark bg + white dots
bluePattern1/.style={
  fill=Blue60!80!black,
  draw=Blue60!80!black,
  postaction={pattern={Dots[distance=2pt,radius=0.6pt]}, pattern color=white}
},
  % 2. Light bg + dark diagonal lines
  bluePattern2/.style={
    fill=Blue60!40,
    draw=Blue60!80!black,
    postaction={pattern=north east lines, pattern color=Blue60!90!black}
  },
  % 3. Medium bg + black crosshatch
  bluePattern3/.style={
    fill=Blue60!65,
    draw=Blue60!80!black,
    postaction={pattern=crosshatch, pattern color=black}
  },
  % 4. Solid bright blue (for contrast)
  bluePattern4/.style={
    fill=Blue60!75!black,
    draw=Blue60!80!black
  },
   bluePattern5Struct/.style={
    fill=Blue60!90,
    draw=Blue60!80!black
  },
 bluePattern6/.style={
    fill=Blue60!35,
    draw=Blue60!80!black
  },
bluePattern7/.style={
  fill=Blue60!10,                % light blue background
  draw=Blue60!80!black,          % dark outline
  postaction={
    pattern=horizontal lines,        % overlay horizontal stripes
    pattern color=Blue60!90!black  % dark blue lines
  }
},

  bluePattern8/.style={
    fill=Blue60!20,
    draw=Blue60!80!black,
    postaction={pattern=dots, pattern color=Blue60!90!black}
  },
  % 6. Medium bg + horizontal lines
  bluePattern9/.style={
    fill=Blue60!60,
    draw=Blue60!80!black,
    postaction={pattern=horizontal lines, pattern color=Blue60!90!black}
  }
}

\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
  ybar=0pt,
  bar width=8pt,
  width=0.52\textwidth, height=4.4cm,
  ymin=0, ymax=100,
  ytick={0,20,40,60,80,100},
  symbolic x coords={P1,P2,P3,P4,P5,P6},
  xtick=data,
  grid=major,
  title={Six Green Variants (solid + patterned)},
  legend style={at={(0.5,-0.20)}, anchor=north, legend columns=2,
    /tikz/every even column/.style={column sep=0.4cm}}
]
  % Bars
\addplot[bluePattern1] coordinates {(P3,72)};
\addplot[bluePattern2] coordinates {(P3,72)};
\addplot[bluePattern3] coordinates {(P3,72)};
\addplot[bluePattern4] coordinates {(P3,72)};
\addplot[bluePattern5] coordinates {(P3,72)};
\addplot[bluePattern6] coordinates {(P3,72)};
\addplot[bluePattern7] coordinates {(P3,72)};
\addplot[bluePattern8] coordinates {(P3,72)};
\addplot[bluePattern9] coordinates {(P3,72)};

\addlegendimage{ybar, bluePattern1}\addlegendentry{dark bg + white dots}
\addlegendimage{ybar, bluePattern2}\addlegendentry{light bg + dark lines}
\addlegendimage{ybar, bluePattern3}\addlegendentry{medium bg + crosshatch}
\addlegendimage{ybar, bluePattern4}\addlegendentry{solid bright blue}
\addlegendimage{ybar, bluePattern5}\addlegendentry{light bg + dark dots}
\addlegendimage{ybar, bluePattern6}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, bluePattern7}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, bluePattern8}\addlegendentry{medium bg + horiz lines}
\addlegendimage{ybar, bluePattern9}\addlegendentry{medium bg + horiz lines}

\end{axis}
\end{tikzpicture}
\caption{Six distinct blue fill styles for print and digital contrast.}
\end{figure}

